Dynamics of niche construction in adaptable populations evolving in diverse environments

In both natural and artificial studies, evolution is often seen as synonymous to natural selection. Individuals evolve under pressures set by environments that are either reset or do not carry over significant changes from previous generations. Thus, niche construction (NC), the reciprocal process to natural selection where individuals incur inheritable changes to their environment, is ignored. Arguably due to this lack of study, the dynamics of NC are today little understood, especially in real-world settings. In this work, we study NC in simulation environments that consist of multiple, diverse niches and populations that evolve their plasticity, evolvability and niche-constructing behaviors. Our empirical analysis reveals many interesting dynamics, with populations experiencing mass extinctions, arms races and oscillations. To understand these behaviors, we analyze the interaction between NC and adaptability and the effect of NC on the population's genomic diversity and dispersal, observing that NC diversifies niches. Our study suggests that complexifying the simulation environments studying NC, by considering multiple and diverse niches, is necessary for understanding its dynamics and can lend testable hypotheses to future studies of both natural and artificial systems.

==> algs/evolution_short.tex <==
\begin{algorithm}
\caption{evolution with niche construction (NC)}
\label{alg:evolution}
\begin{algorithmic}[1]
\State \textbf{Input:} $\mathcal{K},\mathcal{N},\mathcal{G},\epsilon,S$

\State $\mathcal{K}$.initializeGenomes()

\For{$n \in \mathcal{N}$}

\State $i_n=i_0 + \epsilon \cdot n$ \Comment{Initialize intrinsic state}
\State $b_n=0 $ \Comment{Initialize niche-constructed state}
\EndFor


\For{$g  \in \mathcal{G}$}

    \State $\{\sum_{k \in \mathcal{K}_n} a_k | n \in \mathcal{N} \}=\mathcal{K}$.reproduce($\mathcal{N},S,g$) \Comment{Reproduction routine returns the amount of NC per niche}

    \State $\mathcal{N}$.updateNiches($\{\sum_{k \in \mathcal{K}_n} a_k | n \in \mathcal{N} \}$ ) \Comment{Update environmental state of all niches based on NC}

\EndFor
\end{algorithmic}
\end{algorithm}

==> algs/reproduction.tex <==
\begin{algorithm}
\caption{reproduce}
\label{alg:reproduce}
\begin{algorithmic}[1]
\State \textbf{Input:} $\mathcal{K}, \mathcal{N}, S, g$ \Comment{$S\in \{local, global\}$}
\State 
\If{$S ==$ local} \Comment{local competition}
    \State $\text{population} = \{\mathcal{K}.\text{survive}(n)~|~ n\in \mathcal{N}\}$ \Comment{See Eq~\ref{eq:survive_niche}}
    \State $\text{capacity} = \{c_n^g~|~n\in \mathcal{N}\}$
\Else \Comment{Global competition}
    \State $\text{population} = \{\mathcal{K}\}$ \Comment{global competition}
    \State $\text{capacity} = \{\sum_{n\in \mathcal{N}} c_n^g\}$
\EndIf

\State population.order() \Comment{Order the population of each niche based on fitness}
\State 
\For{$\text{p, c} \in \text{zip(population, capacity)}$} \Comment{For each population with its own capacity}
\State $size=0$
\State $\sum_{k \in population} a_k = 0$ \Comment{Variable to keep track of niche construction in this niche}
\While{$\text{size} < c$}
\State p = p[:capacity] \Comment{Drop agents that do not fit in the niche}
\State offspring = p.mate(select)
\State $\sum_{k \in population} a_k \mathrel{+}= p.a + select.a$ \Comment{The NC gene is expressed and modifies the niche}
\State offspring.mutate() \Comment{Eq~\ref{eq:mutation}}
\State $\text{size} \gets \text{size} + 1$
\EndWhile
\EndFor
\State return $\{\sum_{k \in \mathcal{K}_n} a_k | n \in \mathcal{N} \}$

% \If{S $==$ F-selection}
%     \State K.rank()
%     \State $K^{'} = \{ \}$ 
%     \While{$K^{'} < c_{\text{total}}$}
%         \State offspring=k.mate(prob=k.fitness)
%         \State offspring.mutate()
%         \State $K^{'}$.append(offspring)
%     \EndWhile
% \EndIf
% \If{S $==$ N-selection or S $==$ NF-selection}
%     \For{$n \in \{1, \ldots, N\} $}
%     \State $K_n$ = K.survive(n)
%     \If{S $==$ F-selection}
%          \State $K_n$.rank()
%     \Else
%         \State $K_n$.shuffle()
%     \EndIf
%     \State $K^{'}_n = \{ \}$ 
%     \While{$K^{'}_n < c_{n}$}
%         \If{S $==$ NF-selection}
%              \State offspring=k.mate(prob=k.fitness)
%         \Else
%             \State offspring=k.mate(prob=1)
%         \EndIf
        
%         \State offspring.mutate()
%         \State $K^{'}_n$.append(offspring)
%     \EndWhile
%     \EndFor
% \EndIf
\end{algorithmic}
\end{algorithm}

==> sections/results_old.tex <==
\section{Results}

\subsection{Niche construction promotes adaptability}

Under F-selection in Figure \ref{fig:evolution_F} we get:  higher plasticity and a bit higher dispersal and a bit higher genomic diversity that then disappears. There is also variation in the preferred state.

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{images/evolution_F.pdf}
    \caption{Evolution under F-selection}
    \label{fig:evolution_F}
\end{figure}

Under NF-selection in Figure \ref{fig:evolution_NF} we get: higher evolvability, higher diversity. The preferred niche does not show much variation.

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{images/evolution_NF.pdf}
    \caption{Evolution under NF-selection}
    \label{fig:evolution_NF}
\end{figure}

In both Figures \ref{fig:evolution_F} and \ref{fig:evolution_NF} we see that NC causes climatic variability (first row) but these plots are average across trials and NC behaves differently across trials, so now we study plots of a single trial.



\subsection{Fitness-based selection leads to long-distance imigration}

In Figure \ref{fig:F_trial} we analyze the evolution of niche construction in two different trials under F-selection. We observed that trials belonged to one of two categories: the population migrated either in the south (preferred state is 1) or to the north (preferred state is 0). We therefore present plots for two representative trials. For south imigration, we observe that there is some negative NC followed by positive NC with some oscillations. For north immigration, there is only negative NC. I think there is a positive feedback loop here: if the population starts reducing the climate (negative NC) then it starts preferring niches with lower climate which creates a drive to niche-construct negatively. Same goes for positive NC. But in both cases NC is bounded, it does not exceed a certain value. For negative NC this is probably because too much negative NC will cause extinction due to reducing the capacity. In the case of positive NC it is less obvious. What we see is that the population stops adapting its preferred niche as soon as it reaches the end of the map. We can also see that the variance under positive NC increases and this means that there is lack of coordination in NC. Perhaps what is stopping the population is that they are forced to compete in the same niche.

\begin{figure}
\begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{images/NC_F_trial0}
\end{minipage} \quad
\begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{images/heatmap_F_trial0}
\end{minipage}
\begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{images/NC_F_trial2}
\end{minipage} \quad
\begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{images/heatmap_F_trial2}
\end{minipage}
\begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{images/heatmap_F_trial0_variance}
\end{minipage}
\caption{Evolution of niche construction and heatmap for F-selection (Top) a trial where the population migrated to the south (Bottom)a trial where the population migrated to the north}
\label{fig:F_trial}
\end{figure}

\subsection{Niche-limited competition leads to coordination}

Under NF-selection (results in Figure \ref{NF_trial})  we observe that the population goes through cycles of positive and negative niche construction. The population disperses in almost all niches, so NC happens everywhere. Positive NC happens in the south, while negative NC happens on all latitudes. We also observed that variance in NC within niches is much smaller compared to under F-selection. So what could be happening is that introducing niche-limited competition makes it easier for the population to coordinates its NC (because it can do so within a single niche). So niche-limited competition causes plasticity (we know this from the previous paper) and this enable coordination of NC so that the agents do not need to adapt their preferred niche and migrate to the end of the world (mu experiences small oscillations but does not saturate to a high or low value like under F-selection). This means that in this case segregation was achieved.

\begin{figure}
\begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{images/NC_NF_trial4}
\end{minipage} \quad
\begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{images/heatmap_NF_trial4_positive}
\end{minipage}
\begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{images/heatmap_NF_trial4_negative}
\end{minipage}
\begin{minipage}[t]{0.45\columnwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{images/heatmap_NF_trial4_variance}
\end{minipage}
\caption{Evolution of niche construction and heatmap for NF-selection (Top) a trial where the population migrated to the south (Bottom)a trial where the population migrated to the north}
\label{fig:NF_trial}
\end{figure}

Why is NC limited?
Under F-selection maybe it's the fact that the agents cannot go anywhere. Moving was their way of solving the problem of lack of coordination. So it is hard to coordinate and they cancel each other.
Under NF-selection the agents can coordinate but they can also move around thanks to the much higher evolvability. So maybe it is this movement and the fact that niches are sometimes positive and sometimes negative that stops NC. When we look at the behavior in a single niche we see that NC becomes very high and variance is low.

\subsection{Niche construction is inevitable}

In the above experiments we saw that NC is never 0. This creates the hypothesis that NC=0 is not a stable point: even if we enforce it in the population it will not last for long. We now test whether this happens in a controlled experiment: at generation 500 we set all NC genes to 0 until generation 200. This experiment serves also as a causality analysis on NC: is NC causing plasticity?

In Figure \ref{fig:control} we observe that: a) under both selection mechanisms NC returns to increasing at generation 700. This suggests it is not a stable point b) we see that the plasticity under NF-selection decreases from 500 to 700 a bit. But evolvability remains high. There is also a decrease in extinctions, which indicates that NC construction was causing climate variability that was causing extinctions. Under F-selection we see no change. I also looked at where the agents are and they did not change their location (they stay at the north niches). In the case of NF-selection the lower plasticity does not lead to a decrease in dispersal, arguably due to the high evolvability. I am running longer with a longer pause (400 generations) to see the same effects but more pronounced in case I missed something

\begin{figure}
    \centering
    \includegraphics{images/control_trial7}
    \caption{Caption}
    \label{fig:control}
\end{figure}

\subsection{Spatial heterogeneity is necessary for sustainable niche construction}

We now examine what happens when there is a single niche. In Figure \ref{fig:one_niche} we observe that there is a mass extinction. Plasticity and evolvability have risen a lot but the effect on climate is huge so they cannot catch up and there are cycles of big extinctions until everyone dies.


\begin{figure}
    \centering
    \includegraphics{images/one_niche}
    \caption{Evolution of niche construction in a single niche. There is a mass extinction}
    \label{fig:one_niche}
\end{figure}


